The Costs and Benefits of Sharing: Sequential Individual Rationality and Sequential Fairness

In designing dynamic shared service systems that incentivize customers to opt for shared rather than exclusive service, the traditional notion of individual rationality may be insufficient, as a customer's estimated utility could fluctuate arbitrarily during their time in the shared system, as long as their realized utility at service completion is not worse than that for exclusive service. In this work, within a model that explicitly considers the "inconvenience costs" incurred by customers due to sharing, we introduce the notion of sequential individual rationality (SIR) that requires that the disutility of existing customers is nonincreasing as the system state changes due to new customer arrivals. Next, under SIR, we observe that cost sharing can also be viewed as benefit sharing, which inspires a natural definition of sequential fairness (SF) - the total incremental benefit due to a new customer is shared among existing customers in proportion to the incremental inconvenience suffered. We demonstrate the effectiveness of these notions by applying them to a ridesharing system, where unexpected detours to pick up subsequent passengers inconvenience the existing passengers. Imposing SIR and SF reveals interesting and surprising results, including: (a) natural limits on the incremental detours permissible, (b) exact characterization of "SIR-feasible" routes, which boast sublinear upper and lower bounds on the fractional detours, (c) exact characterization of sequentially fair cost sharing schemes, which includes a strong requirement that passengers must compensate each other for the detour inconveniences that they cause, and (d) new algorithmic problems related to and motivated by SIR.

==> full/abstract.tex <==
\begin{abstract}
In designing cost sharing schemes for dynamic shared service systems that incentivize customers to opt for shared service rather than exclusive service, the traditional notion of individual rationality may be insufficient, as it allows for a customer's estimated utility to fluctuate arbitrarily \textit{during} their time in the system, as long as their actual utility at the time of service completion is not worse than that for exclusive service. In this work, within a model that explicitly takes into account the ``inconvenience costs'' incurred by customers due to sharing, we introduce the notion of \textit{sequential} individual rationality (SIR) that requires that the disutility (the sum of monetary and inconvenience costs) of existing customers is nonincreasing as the system state changes due to new customer arrivals. Next, we observe that under any budget-balanced, SIR cost sharing scheme, the total amount by which the customers' disutilities decrease (which can be viewed as the total incremental benefit due to sharing) is a constant. This observation inspires a ``dual'' notion of viewing cost sharing schemes as \textit{benefit sharing schemes}, under which we introduce a natural definition of \textit{sequential} fairness (SF)---the total incremental benefit due to the arrival of a new customer is (partly) shared among the existing customers in proportion to the incremental inconvenience costs they suffer as a result.

We demonstrate the effectiveness of these notions by applying them to a ridesharing system, where unexpected detours taken to pick up subsequent passengers inconvenience the existing passengers. Imposing SIR and SF on the routing and cost sharing schemes for ridesharing reveals interesting and surprising results: (a)~the SIR constraints induce a natural limit on the incremental detours permissible as the ride progresses, (b)~we provide an exact characterization of all routes for which there exists some cost sharing scheme that is SIR on that route, and under these constraints, for realistic scenarios, we also show a $\Theta(\sqrt{n})$ upper bound and a $\Theta(\log n)$ lower bound on the total detour experienced by the passengers as a fraction of the shortest distance to their destination, (c)~we also provide an exact characterization of sequentially fair cost sharing schemes, which brings out several useful structural properties, including a strong requirement that \textit{passengers must compensate each other for the detour inconveniences that they cause}, and finally, (d)~we conclude with an extended discussion of new algorithmic problems related to and motivated by sequential individual rationality, and important future work.
\end{abstract} 
